Learning Dense Representations of Phrases at Scale

Open-domain question answering can be reformulated as a phrase retrieval problem, without the need for processing documents on-demand during inference (Seo et al., 2019). However, current phrase retrieval models heavily depend on sparse representations and still underperform retriever-reader approaches. In this work, we show for the first time that we can learn dense representations of phrases alone that achieve much stronger performance in open-domain QA. We present an effective method to learn phrase representations from the supervision of reading comprehension tasks, coupled with novel negative sampling methods. We also propose a query-side fine-tuning strategy, which can support transfer learning and reduce the discrepancy between training and inference. On five popular open-domain QA datasets, our model DensePhrases improves over previous phrase retrieval models by 15%-25% absolute accuracy and matches the performance of state-of-the-art retriever-reader models. Our model is easy to parallelize due to pure dense representations and processes more than 10 questions per second on CPUs. Finally, we directly use our pre-indexed dense phrase representations for two slot filling tasks, showing the promise of utilizing DensePhrases as a dense knowledge base for downstream tasks.

==> tables/slot_filling_dev.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{1.2cm}{\textbf{Model}}& \multicolumn{2}{c}{\textbf{T-REx}} & \multicolumn{2}{c}{\textbf{ZsRE}} \\\cmidrule{2-3} \cmidrule{4-5}
        & Accuracy & F1 & Accuracy & F1 \\
        \midrule

        BART &  43.84 & 48.25 & 3.03 & 12.61 \\
        T5 & 47.24 & 51.73 & 1.58 & 10.80 \\
        BERT + DPR &  - & - & - & - \\
        BART + DPR &  56.70 & 60.19 & 34.96 & 44.79 \\
        RAG & 61.48 & 65.03 & 47.42 & 57.98 \\
        \midrule
        \ours~(+ NQ) & 22.76 & 28.35 & 30.32 & 35.74 \\
        \ours~(+ 5K) & 46.86 & 58.81 & 28.41 & 50.86 \\
        \ours~(+ 10K) & - & - & - & - \\
        \bottomrule
    \end{tabular}
    }
    \caption{Slot filling task results on the T-REx and Zero shot RE (ZsRE) development sets.\jinhyuk{Maybe try test set in KILT web server}
    \label{tab:re}}
\end{table}

